State Derivative Normalization for Continuous-Time Deep Neural Networks

The importance of proper data normalization for deep neural networks is well known. However, in continuous-time state-space model estimation, it has been observed that improper normalization of either the hidden state or hidden state derivative of the model estimate, or even of the time interval can lead to numerical and optimization challenges with deep learning based methods. This results in a reduced model quality. In this contribution, we show that these three normalization tasks are inherently coupled. Due to the existence of this coupling, we propose a solution to all three normalization challenges by introducing a normalization constant at the state derivative level. We show that the appropriate choice of the normalization constant is related to the dynamics of the to-be-identified system and we derive multiple methods of obtaining an effective normalization constant. We compare and discuss all the normalization strategies on a benchmark problem based on experimental data from a cascaded tanks system and compare our results with other methods of the identification literature.

==> fig/fig_rknn_v3.tex <==
\begin{tikzpicture}[thick, scale=0.8]

	% Blocks
	\node [input, name=inputx] {};
	% \node [input, right of=inputxlow, node distance=3cm, name=inputu] {};
	
	% first
	\node [blockNN, right of=inputx, node distance=1cm] (NN1) % {\includegraphics[scale=0.19]{fig/Netzwerk1_Titelbild}};
	{$f_{_{\text{NN}}}$};
    \draw [->] (inputx) -- node[above]{$\hat{x}_n$} (NN1);
    
    \node [blockConst, right of=NN1, node distance=1.2cm] (h1) {$\frac{h}{2}$};
	\draw [->] (NN1) -- (h1);
    
	\node [ring, right of=h1, node distance=0.8cm] (sum1) {$\sum$};
	\draw [->] (h1) -- (sum1);
	
	
	% second
	\node [blockNN, right of=sum1, node distance=1cm] (NN2) % {\includegraphics[scale=0.19]{fig/Netzwerk1_Titelbild}};
	{$f_{_{\text{NN}}}$};
    \draw [->] (sum1) -- (NN2);
    
    \node [blockConst, right of=NN2, node distance=1.2cm] (h2) {$\frac{h}{2}$};
	\draw [->] (NN2) -- (h2);
    
	\node [ring, right of=h2, node distance=0.8cm] (sum2) {$\sum$};
	\draw [->] (h2) -- (sum2);
	
	
	
	% third
	\node [blockNN, right of=sum2, node distance=1cm] (NN3) % {\includegraphics[scale=0.19]{fig/Netzwerk1_Titelbild}};
	{$f_{_{\text{NN}}}$};
    \draw [->] (sum2) -- (NN3);
    
    \node [blockConst, right of=NN3, node distance=1.2cm] (h3) {$h$};
	\draw [->] (NN3) -- (h3);
    
	\node [ring, right of=h3, node distance=0.8cm] (sum3) {$\sum$};
	\draw [->] (h3) -- (sum3);
	
	
	
    % fourth
	 \node [blockNN, right of=sum3, node distance=1cm] (NN4) % {\includegraphics[scale=0.19]{fig/Netzwerk1_Titelbild}};
	 {$f_{_{\text{NN}}}$};
     \draw [->] (sum3) -- (NN4);
    
	\node [ring, right of=NN4, node distance=1cm] (sum4) {$\sum$};
	\draw [->] (NN4) -- (sum4);
	
	\node [blockConst, right of=sum4, node distance=0.8cm] (h4) {$\frac{h}{6}$};
	\draw [->] (sum4) -- (h4);
    
	\node [ring, right of=h4, node distance=0.8cm] (sum5) {$\sum$};
	\draw [->] (h4) -- (sum5);
	
	\node [input, right of=sum5, node distance=1.5cm] (out) {};
	\draw [->] (sum5) -- node[above]{$\hat{x}_{n+1}$}(out);
	
	
	

	
	
	% low x sum
	\node [input, right of=inputx, node distance=0.3cm, name=x1] {};
	\node [input, below of=x1, node distance=0.8cm, name=x2] {};
	\draw [-] (x1) -- (x2);
	\draw [->] (x2) -| (sum1);
	\draw [->] (x2) -| (sum2);
	\draw [->] (x2) -| (sum3);
	\draw [->] (x2) -| (sum5);
	
	% low u
	\node [input, below of=inputx, node distance=1.6cm, name=u1] {};
	\draw [->, blue] (u1) -| node[above left]{$u_n$}(NN1);
	\draw [->, blue] (u1) -| (NN2);
	\draw [->, blue] (u1) -| (NN3);
	\draw [->, blue] (u1) -| (NN4);
	
    % output network
	 \node [blockNN, below of=sum5, node distance=1.6cm] (NN5) % {\includegraphics[scale=0.19]{fig/Netzwerk1_Titelbild}};
	 {$h_{_{\text{NN}}}$};
    \node [input, below of=out, node distance=1.6cm] (outy) {};
    
	\draw [->] (NN5) -- node[above]{$\hat{y}_{n}$}(outy);
	\draw [->] (x2) -| (NN5);
	\draw [->, blue] (u1) -- (NN5);
	
	
	% upper k
	\node [input, right of=NN1, node distance=0.7cm, name=k1] {};
	\node [input, right of=NN2, node distance=0.7cm, name=k2] {};
	\node [input, right of=NN3, node distance=0.7cm, name=k3] {};

	\node [input, above of=sum4, node distance=1cm, name=t1] {};
	\node [input, above of=sum4, node distance=1.5cm, name=t2] {};
	\node [input, above of=sum4, node distance=2cm, name=t3] {};
	
	\node [input, left of=t1, node distance=0.8cm, name=s1] {};
	\node [input, left of=t2, node distance=0.8cm, name=s2] {};
	\node [input, left of=t3, node distance=0.8cm, name=s3] {};
	
	\node [blockConst, left of=s1, node distance=2cm] (sh1) {$2$};
	\node [blockConst, left of=s2, node distance=4cm] (sh2) {$2$};
	
	\draw [->] (s1) -- (sum4);
	\draw [->] (s2) -- (sum4);
	\draw [->] (s3) -- (sum4);
	
	\draw [-] (sh1) -- (s1);
	\draw [-] (sh2) -- (s2);
	\draw [-] (k1) |- (s3);
	
	\draw [->] (k2) |- (sh2);
	\draw [->] (k3) |- (sh1);
	
\end{tikzpicture}

==> fig/fig_tdn_disc.tex <==

        \begin{tabular}{l}
            \begin{tikzpicture}
                \begin{axis}[
                    axis y line = left,
                    axis x line = bottom,
                    grid=major,
                    width=0.8\linewidth,
                    height=0.2\linewidth,
                    % at={(0\fwidth,0\fheight)},
                    scale only axis,
                    % xmin=0,
                    % xmax=1.1,
                    % xtick={0,0.3, 0.6, 0.9, 1.2},
                    % ymin=-0.5,
                    % ymax=1.8,
                    % xlabel style={font=\color{white!15!black}},
                    xlabel={Time in $s$},
                    % ymin=-2000,
                    % ymax=2000,
                    % ytick={1500,1000,...,-1500},
                    % yticklabels={1.5,1,0.5,0,-0.5,-1,-1.5},
                    % ylabel style={font=\color{white!15!black}},
                    ylabel style={align=center}, 
                    ylabel = {Output [V]},
                    % axis background/.style={fill=white},
                    % xmajorgrids,
                    % ymajorgrids,
                    % legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
                ]
\addplot [color=black, mark=o]
  table[row sep=crcr]{%
0	5.20500495918212\\
20	5.20012207217517\\
40	5.21782253757534\\
60	5.20744640268559\\
80	5.30266269932097\\
100	5.40825513084611\\
120	5.53032730601968\\
140	5.74151216906996\\
160	5.92095826657511\\
180	5.99786373693446\\
200	6.02349889372091\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
0	5.20500495918212\\
5	5.20012207217517\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
20	5.20012207217517\\
25	5.21782253757534\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
40	5.21782253757534\\
45	5.20744640268559\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
60	5.20744640268559\\
65	5.30266269932097\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
80	5.30266269932097\\
85	5.40825513084611\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
100	5.40825513084611\\
105	5.53032730601968\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
120	5.53032730601968\\
125	5.74151216906996\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
140	5.74151216906996\\
145	5.92095826657511\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
160	5.92095826657511\\
165	5.99786373693446\\
        };
        \addplot [color=red, mark=o]
  table[row sep=crcr]{%
180	5.99786373693446\\
185	6.02349889372091\\
        };
                \end{axis}
            \end{tikzpicture}
        \end{tabular}


==> fig/results_data.tex <==
trained
exp1 run1:
  dt_model: 0.03601381225019065
  final_test_metric: 0.21508142837657962
exp1 run10:
  dt_model: 0.05743698807027829
  final_test_metric: 0.22367286452952914
exp1 run2:
  dt_model: 0.04591468288497492
  final_test_metric: 0.26862603757805026
exp1 run3:
  dt_model: 0.16536223612354775
  final_test_metric: 0.5965899983131618
exp1 run4:
  dt_model: 0.05148473973935558
  final_test_metric: 0.24667747418833447
exp1 run5:
  dt_model: 0.039487525099253865
  final_test_metric: 0.22126251437001204
exp1 run6:
  dt_model: 0.16759336945152847
  final_test_metric: 0.4785843093049573
exp1 run7:
  dt_model: 0.050398511212550776
  final_test_metric: 0.21841382919276506
exp1 run8:
  dt_model: 0.04653553371138462
  final_test_metric: 0.20546747610595167
exp1 run9:
  dt_model: 0.05480241063801218
  final_test_metric: 0.3025792644983298

a = np.array([0.03601381225019065, 0.05743698807027829, 0.04591468288497492, 0.16536223612354775, 0.05148473973935558, 0.039487525099253865, 0.16759336945152847, 0.050398511212550776, 0.04653553371138462, 0.05480241063801218 ])
>>> np.mean(a)
0.07150298091810771
>>> np.std(a)
0.047883626951625666

10 reps
  all exp mean: 0.29769551964576707
  all exp std: 0.1258842462798383
  best 0.21508142837657962
  
  
-------------------------------
cross_val
dt model: 0.5428835233189813
20 reps
 - 0.2803139791653193
    - 0.38136809536722893
    - 0.20530225327883864
    - 0.27542917085871677
    - 0.31882532047048434
    - 0.2824022290857308
    - 0.2913141838560751
    - 0.31746071175212137
    - 0.23377579403554768
    - 0.265709333894929
  - - 0.22074482501797968
    - 0.32989449592064707
    - 0.2896904178475634
    - 0.20978775598780008
    - 0.24542796853210974
    - 0.3984876694534261
    - 0.2453103796488067
    - 0.29062419240937865
    - 0.2493183836780409
    - 0.22297616615734692
    
    

 import numpy as np
 a = np.array([ 0.2803139791653193,0.38136809536722893,0.20530225327883864,0.27542917085871677,0.31882532047048434,0.2824022290857308,0.2913141838560751,0.31746071175212137,0.23377579403554768,0.265709333894929,0.22074482501797968,0.32989449592064707,0.2896904178475634,0.20978775598780008,0.24542796853210974,0.3984876694534261,0.2453103796488067,0.29062419240937865,0.2493183836780409,0.22297616615734692])
 np.mean(a)
 0.2777081663209045
 np.std(a)
 0.051441594502518874
np.min(a) 
0.20530225327883864
 
 
 
 --------------------------------------
 bla
 dt model:
 0.05361930294906166
10 reps
  all exp mean: 0.26333777598786323
  all exp std: 0.028407201714353687
  best 0.22528847831489773
